An Attention-based Representation Distillation Baseline for Multi-Label Continual Learning

The field of Continual Learning (CL) has inspired numerous researchers over the years, leading to increasingly advanced countermeasures to the issue of catastrophic forgetting. Most studies have focused on the single-class scenario, where each example comes with a single label. The recent literature has successfully tackled such a setting, with impressive results. Differently, we shift our attention to the multi-label scenario, as we feel it to be more representative of real-world open problems. In our work, we show that existing state-of-the-art CL methods fail to achieve satisfactory performance, thus questioning the real advance claimed in recent years. Therefore, we assess both old-style and novel strategies and propose, on top of them, an approach called Selective Class Attention Distillation (SCAD). It relies on a knowledge transfer technique that seeks to align the representations of the student network -- which trains continuously and is subject to forgetting -- with the teacher ones, which is pretrained and kept frozen. Importantly, our method is able to selectively transfer the relevant information from the teacher to the student, thereby preventing irrelevant information from harming the student's performance during online training. To demonstrate the merits of our approach, we conduct experiments on two different multi-label datasets, showing that our method outperforms the current state-of-the-art Continual Learning methods. Our findings highlight the importance of addressing the unique challenges posed by multi-label environments in the field of Continual Learning. The code of SCAD is available at https://github.com/aimagelab/SCAD-LOD-2024.

==> contents/scad_algorithm.tex <==
\begin{algorithm}[H]
\caption{SCAD algorithm}\label{alg:scad}
\setstretch{1.2}
\begin{algorithmic}
\Require Intermediate representations $F_\mathcal{T}$, $F_\mathcal{S}$, number of tokens $N$, weights $W_1$, $W_2$,\\\hspace{3.3em}biases $b_1$, $b_2$, adapter layers $\mathcal{L}$
\State $loss_\text{\,FP} \gets 0$
\For{$l\:\textbf{in}\:\mathcal{L}$}
\State $norm\_F_\mathcal{T} \gets F_\mathcal{T}^l / ||F_\mathcal{T}^l||_2^2$
\State $norm\_F_\mathcal{S} \gets F_\mathcal{S}^l / ||F_\mathcal{S}^l||_2^2$
\State $\mathcal{R}_\mathcal{T} \gets norm\_F_\mathcal{T} \cdot norm\_F_\mathcal{T}^T $
\State $\mathcal{R}_\mathcal{S} \gets norm\_F_\mathcal{S} \cdot norm\_F_\mathcal{S}^T $
\State $attn\_vec_\mathcal{T} \gets \mathcal{R}_\mathcal{T}\left[ 0,1:N+1 \right]$
\State $attn\_vec_\mathcal{S} \gets \mathcal{R}_\mathcal{S}\left[ 0,1:N+1 \right]$

\State $bin\_vec \gets gumbel(stack(attn\_vec_\mathcal{T} \odot W_1 + b_1, attn\_vec_\mathcal{T} \odot W_2 + b_2))$

\State $dist \gets bin\_vec \odot (attn\_vec_\mathcal{T} - attn\_vec_\mathcal{S})^2$
\State $loss_\text{\,FP} \gets loss_\text{\,FP} + mean(dist)$
\EndFor
\State $\mathcal{L}_\text{FP} \gets \lambda_\text{FP} \cdot \frac{1}{|L|} loss_\text{\,FP}$

\end{algorithmic}
\end{algorithm}

==> contents/sup_hyp_tables.tex <==

 \begin{table}[H]
    \centering
    \caption{Hyperparameters used for the IIRC-CIFAR100 benchmark.}
    % \resizebox{.42\paperheight}{!}{%
    \begin{tabular}{ccl}%@{\hskip 0.5cm}
    \noalign{\smallskip}
    \hline
    \noalign{\smallskip}

\multicolumn{3}{c}{\textbf{IIRC CIFAR100 - Class-IL}}\\\noalign{\smallskip}
    \hline
    \noalign{\smallskip}
\textit{shared} & &  $\text{Eps}: 5$ $\text{bs}: 16$ \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\textbf{Method} & \textbf{Buffer size} & \textbf{Other parameters} \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
JOINT & - &$\text{lr}:0.03$ \\
SGD & - &$\text{lr}:0.03$ \\
L2P \cite{wang2022learning} & - &$\text{lr}:0.03$ $\;\text{pool\_size}: 10$ \\
CP \cite{smith2022coda} & - &$\text{lr}:0.001$ $\;\text{pool\_size}: 100$\\
ER \cite{ratcliff1990connectionist,robins1995catastrophic} & $500$ &$\text{lr}:0.03$ \\
  & $2000$ &$\text{lr}:0.03$ \\
ER-ACE \cite{caccia2022new} & $500$ &$\text{lr}:0.03$ \\
  & $2000$ &$\text{lr}:0.03$ \\
\dpp \cite{buzzega2020dark} & $500$ &$\text{lr}:0.03$ $\alpha:0.3$ $\beta:0.8$ \\
  & $2000$ &$\text{lr}:0.03$ $\alpha:0.3$ $\beta:0.8$ \\
\methnam & $500$ &$\text{lr}:0.03$ $\alpha:0.3$ $\beta:0.8$ $\lambda_\text{FP}:1.0$ $\lambda_{\text{FP\_rep}}:0.1$ $\mathcal{L}:\{1,4,7,10\}$ \\
  & $2000$ &$\text{lr}:0.03$ $\alpha:0.3$ $\beta:0.8$ $\lambda_\text{FP}:1.0$ $\lambda_{\text{FP\_rep}}:0.1$ $\mathcal{L}:\{1,4,7,10\}$ \\
\noalign{\smallskip}
    \hline
    \noalign{\smallskip}
    \end{tabular}
    
    % }
\label{tab:sup_hyp_iirc}
\end{table}

\clearpage

 \begin{table}[H]
    \centering
    \caption{Hyperparameters used for the WebVision benchmark.}
    % \resizebox{.42\paperheight}{!}{%
    
    \begin{tabular}{ccl}%@{\hskip 0.5cm}
\noalign{\smallskip}
    \hline
    \noalign{\smallskip}
    
\multicolumn{3}{c}{\textbf{WebVision - Class-IL}}\\\noalign{\smallskip}
    \hline
    \noalign{\smallskip}
\textit{shared} &&  $\text{Eps}: 1$ $\text{bs}: 16$ \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\textbf{Method} & \textbf{Buffer size} & \textbf{Other parameters} \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
JOINT & - &$\text{lr}:0.03$ \\
SGD & - &$\text{lr}:0.03$ \\
L2P \cite{wang2022learning} & - &$\text{lr}:0.03$ $\;\text{pool\_size}: 10$ \\
CP \cite{smith2022coda} & - &$\text{lr}:0.001$ $\;\text{pool\_size}: 100$ \\
ER \cite{ratcliff1990connectionist,robins1995catastrophic} & $2000$ &$\text{lr}:0.03$ \\
  & $5000$ &$\text{lr}:0.03$ \\
ER-ACE \cite{caccia2022new} & $2000$ &$\text{lr}:0.03$ \\
  & $5000$ &$\text{lr}:0.03$ \\
\dpp \cite{buzzega2020dark} & $2000$ &$\text{lr}:0.03$ $\alpha:0.3$ $\beta:0.9$ \\
  & $5000$ &$\text{lr}:0.03$ $\alpha:0.3$ $\beta:0.9$ \\
\methnam & $2000$ &$\text{lr}:0.03$ $\alpha:0.3$ $\beta:0.9$ $\lambda_\text{FP}:1.0$ $\lambda_{\text{FP\_rep}}:0.1$ $\mathcal{L}:\{1,4,7,10\}$ \\
  & $5000$ &$\text{lr}:0.03$ $\alpha:0.3$ $\beta:0.9$ $\lambda_\text{FP}:1.0$ $\lambda_{\text{FP\_rep}}:0.1$ $\mathcal{L}:\{1,4,7,10\}$ \\
\noalign{\smallskip}
    \hline
    \noalign{\smallskip}
    \end{tabular}
    
    % }
    \label{tab:sup_hyp_webvision}
\end{table}
%     \label{tab:hyperpc10}
% \end{table}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
